Constant-Time Inverse Suffix Array Queries in Compact Space and Sublinear-Time Construction of Suffix Array Indexes

For a text $T\in[0..\sigma)^n$ with $2\leq\sigma\leq n$, its suffix array orders the suffix starting positions lexicographically, while its inverse suffix array maps each position to its suffix's rank. Since compressed suffix arrays and FM-indexes appeared in 2000, a central goal has been to support both queries in $O(n\log\sigma)$ bits. Thankachan recently reduced inverse suffix array query time to $O(\log\log n/\log\log\sigma)$, but constant time remained open. We give the first inverse suffix array structure with optimal space and query time: $O(n\log\sigma)$ bits and $O(1)$ time. For binary texts, this unconditionally separates the two queries for deterministic structures, since every $O(n)$-bit suffix array structure in the cell-probe model with $\Theta(\log n)$-bit cells has worst-case query time $\Omega(\log\log n/\log\log\log n)$. Construction is a second challenge: linear time can take $\Theta(\log_{\sigma} n)$ times as long as reading the input or writing a compact index. Previously, sublinear construction was known for only one such index supporting both queries. In the word RAM with $\Theta(\log n)$-bit words, we deterministically construct the new structure and two suffix array families from the packed text in $O(n\min(1,\log\sigma/\sqrt{\log n}))$ time. For $B\geq2$, the first family uses $O(n\log\sigma(1+\log_B\log_\sigma n))$ bits and has query time $O(B(1+\log_B\log_\sigma n))$, whereas the second uses $O(Bn\log\sigma(1+\log_B\log_\sigma n))$ bits and has query time $O(1+\log_B\log_\sigma n)$. Each has peak preprocessing space bounded by its index size. For binary texts, the second family matches the deterministic cell-probe time-space lower bound whenever $B\geq(\log\log n)^{\Omega(1)}$, and, outside the slowest-query regimes, improving the deterministic construction time to $o(n/\sqrt{\log n})$ would yield an equally fast Dictionary Matching algorithm.

==> settings.tex <==

%
\makeatletter
\newcommand{\refcheckize}[1]{%
  \expandafter\let\csname @@\string#1\endcsname#1%
  \expandafter\DeclareRobustCommand\csname relax\string#1\endcsname[1]{%
    \csname @@\string#1\endcsname{##1}\@for\@temp:=##1\do{\wrtusdrf{\@temp}\wrtusdrf{{\@temp}}}}%
  \expandafter\let\expandafter#1\csname relax\string#1\endcsname
}
\newcommand{\refcheckizetwo}[1]{%
  \expandafter\let\csname @@\string#1\endcsname#1%
  \expandafter\DeclareRobustCommand\csname relax\string#1\endcsname[2]{%
    \csname @@\string#1\endcsname{##1}{##2}\wrtusdrf{##1}\wrtusdrf{{##1}}\wrtusdrf{##2}\wrtusdrf{{##2}}}%
  \expandafter\let\expandafter#1\csname relax\string#1\endcsname
}
\makeatother

\refcheckize{\cref}
\refcheckize{\Cref}
\refcheckizetwo{\crefrange}
\refcheckizetwo{\Crefrange}

%
\makeatletter
\renewcommand\thmt@autorefsetup{\@xa\def\csname\thmt@envname autorefname\@xa\endcsname\@xa{\thmt@thmname}}
\makeatother

%
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{proposition}[theorem]{Proposition}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{construction}[theorem]{Construction}
\crefname{construction}{Construction}{Constructions}
\crefname{claim}{Claim}{Claims}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}

%
\AddToHook{env/theorem/begin}{\crefalias{section}{theorem}}
\AddToHook{env/corollary/begin}{\crefalias{theorem}{corollary}}
\AddToHook{env/lemma/begin}{\crefalias{theorem}{lemma}}
\AddToHook{env/fact/begin}{\crefalias{theorem}{fact}}
\AddToHook{env/observation/begin}{\crefalias{theorem}{observation}}
\AddToHook{env/proposition/begin}{\crefalias{theorem}{proposition}}
\AddToHook{env/definition/begin}{\crefalias{theorem}{definition}}
\AddToHook{env/claim/begin}{\crefalias{theorem}{claim}}
\AddToHook{env/construction/begin}{\crefalias{theorem}{construction}}
\AddToHook{env/remark/begin}{\crefalias{theorem}{remark}}
\AddToHook{env/example/begin}{\crefalias{theorem}{example}}

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
\newcommand{\creflastconjunction}{, and\nobreakspace}
\crefname{observation}{Observation}{Observations}
\Crefname{observation}{Observation}{Observations}

%
\definecolor{mypink}{RGB}{199, 21, 133}
\hypersetup{
  colorlinks,
  urlcolor = blue,
  linkcolor = mypink,
  citecolor = blue
}

%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%

%
\setul{2pt}{0.6pt}

%
\setlength{\FrameSep}{1.5ex}

%
\setlist[enumerate]{nosep, topsep=1ex}
\setlist[itemize]{nosep, topsep=1ex}
\setlist[description]{nosep,topsep=1ex}

%
\allowdisplaybreaks

%
\lineskiplimit=-5pt

%
\let\oldabstract\abstract
\let\oldendabstract\endabstract
\makeatletter
\renewenvironment{abstract}
{\renewenvironment{quotation}%
  {\list{}{\addtolength{\leftmargin}{0.4em}%
    \listparindent 1.5em%
     \itemindent    \listparindent%
     \rightmargin   \leftmargin%
     \parsep        \z@ \@plus\p@}%
     \item\relax}%
  {\endlist}%
\oldabstract}
{\oldendabstract}
\makeatother

%
\fxsetup{mode=multiuser,theme=color, layout=inline}
\FXRegisterAuthor{tk}{atk}{\color{red} {\bf Tomasz}}
\FXRegisterAuthor{dk}{adk}{\color{green!70!black} {\bf Dominik}}

%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%

%
\newcommand{\DSComponents}{%
  \vspace{2ex}%
  \noindent%
  \textbf{\textit{Data structure}}\quad%
}
\newcommand{\DSQueries}{%
  \vspace{2ex}%
  \noindent%
  \textbf{\textit{Queries}}\quad%
}
\newcommand{\DSConstruction}{%
  \vspace{2ex}%
  \noindent%
  \textbf{\textit{Construction}}\quad%
}

%
\newenvironment{bfdescription}
  {\begin{description}[style=sameline,itemsep=1ex,font={\normalfont\bf}]}
  {\end{description}\vspace{-1.2ex}}

%
\renewcommand*\descriptionlabel[1]{\hspace\labelsep\normalfont\itshape #1}




